Nonstationary Multivariate Gaussian Processes for Electronic Health Records

We propose multivariate nonstationary Gaussian processes for jointly modeling multiple clinical variables, where the key parameters, length-scales, standard deviations and the correlations between the observed output, are all time dependent. We perform posterior inference via Hamiltonian Monte Carlo (HMC). We also provide methods for obtaining computationally efficient gradient-based maximum a posteriori (MAP) estimates. We validate our model on synthetic data as well as on electronic health records (EHR) data from Kaiser Permanente (KP). We show that the proposed model provides better predictive performance over a stationary model as well as uncovers interesting latent correlation processes across vitals which are potentially predictive of patient risk.

==> original_versions.tex <==


% These are the original sections from Rui's paper for related work and the model presentation. 
% I'm just pasting them here as back up as I make changes in the main document.  



\section{Related Work}
To model multivariate spatial process, separable cross-covariance functions are introduced in $\cite{mardia1993spatial}$. In the geostatistics literature it is introduced as the intrinsic coregionalization model in \cite{goovaerts1997geostatistics}. This model assumes that all component processes share the same structure, which is may not be justifiable in practice. A generalized model is the linear model of regionalization, where the covariance matrix is generalized as the sum of different separable covariance matrices in \cite{wheeler2007assessment}. A more general non-separable kernels are constructed using convolution processes \cite{alvarez2012kernels}. \cite{majumdar2007multivariate} provided a multivariate spatial process using convolved covariance functions, which is treated as a parsimonious approach. The corresponding model for nonstationary setting is discussed in \cite{majumdar2010generalized}. The spatially varying linear model of coregionalization is studied in \cite{gelfand2004nonstationary} through a spatially varying Wishart process. Gneiting et al. \cite{gneiting2010matern} proposed multivariate Matern cross-covariance functions, where each constituent component is a Matern process. The corresponding nonstationary setting is studied in \cite{kleiber2012nonstationary}.


To model the non-stationarity in spatial processes, Brunsdon proposed geographical weighted regression GWR in \cite{brunsdon1996geographically}, which connect the relation between the weight and sample sites. Bayesian regression models with spatially varying coefficient process (SVCP) are proposed in \cite{gelfand2003spatial} where Gaussian process priors are put on coefficients. The main difference of the two approaches is that SVCP is a single statistical model specified in a hierarchical manner while GWR is an ensemble of local spatial regression models. Wheeler compared both models under different levels of collinearities and illustrated SVGP is more robust than GWR in \cite{wheeler2007assessment}. Using kernel convolution, a nonstationary, univariate Matern correlation function is introduced in  \cite{paciorek2004nonstationary} and illustrated in the real data in \cite{paciorek2006spatial} that nonstationary model is marginally better than a stationary model based on hold-out predictive criteria. \cite{paciorek2006spatial} also provide a non-stationary kriging approach which is significantly better than other models with respect to predictive performance. Stein extended the nonstationary kernel by using both spatially varying local geometric anisotropy and the degree of differentiability in \cite{stein2005nonstationary}. Local likelihood estimation is proposed to efficiently estimate parameter.



\section{Multivariate Gaussian Processes}
A Multivariate Gaussian process (MGP) defines a distribution over multivariate functions $\bm f(t) = (f_1(t), \ldots f_M(t))^T$. The general MGP including a measurement error term is  
\begin{align}
    & \bm y(t) = \bm f(t) + \bm\epsilon(t) \,, \qquad \bm \epsilon(t) \sim  \mathcal{N}(0, \sigma^2_{err}I) \nonumber \\
    & \bm f(t) \sim \mathrm{GP}(0, K^f) 
\end{align}
where $K^f$ is a covariance function. For any collection of inputs $t_1, \ldots, t_N$, the function values $\bm f_n = \bm f(t_n)$ follow a multivariate normal distribution
\begin{align}
    \Vec{\bm f} \equiv \mathrm{vec}([\bm f_1, \ldots, \bm f_N]^T) \sim \mathcal{N}(\bm 0, \bm K^f)
\end{align}
where $\mathrm{vec}$ is vectorization operator and the covariance matrix $\bm K^f$ is generated from covariance function $K^f$. Generally, an MGP is separable when a decomposition exists such that given inputs $t, t'$ and dimension indices $m, m'$,  $K^f(t, t', m, m') = B(m, m')K(t, t')$. In matrix notation, it is equivalent to $\bm K^f = \bm B \otimes \bm K$, where covariance matrix $\bm B \in \mathbb{R}^{M \times M}$ summarizes the relation across output dimensions and covariance matrix $\bm K$ summarizes the relation across time separately.

Typically, the dimension size $M$ is much smaller than the data size $N$. $\bm B$ is modeled directly while $\bm K$ is model via kernel functions. Specifically, covariance matrix $\bm B$ is modeled using a Cholesky decomposition such that $\bm B = \bm L \bm L^T$ and $\bm K$ is parametrized by some kernel functions. A commonly used stationary kernel is the square exponential or radial basis function (RBF) kernel
\begin{align}
    k_{\mathrm{RBF}}(t, t') = \sigma^2\exp\left(-\frac{(t - t')^2}{2\ell^2}\right)\,.
\end{align}
where the signal variance $\sigma$ corresponds to the range scale of function and the length-scale encodes how fast the function values can change with respect to the distance $|t - t'|$. 

The separable multivariate Gaussian process has an equivalent representation using the linear model of coregionalization:
\begin{align}
    & \bm y(t) = \bm L \bm g(t) + \bm\epsilon(t)\,, \qquad \bm\epsilon(t) \sim \mathcal{N}(0, \sigma^2_{err}I) \nonumber \\
    & g_d(t) \stackrel{iid}{\sim} \mathrm{GP}(0, K)
\end{align}
They share the same log likelihood such that
\begin{align}
    \ell = \log\mathcal{N}(\vec{\bm y}|0, \bm B\otimes \bm K + \sigma^2_{err}I)
\end{align}
where $\bm B = \bm L^T\bm L$.

The prior of $\sigma^2_{err}$ and $\bm L$ are given as
\begin{align}
    & \sigma^2_{err} \sim \mathrm{IG}(a, b)\,, \nonumber \\
    & L_{ij} \sim \mathcal{N}(0, c) \qquad i\geq j\,.
\end{align}
We put a non-informative prior for $\sigma$ such that $\log\sigma \propto 1$ and an informative prior for length-scale parameter $\ell$ such that $\log\ell \sim \mathcal{N}(0, s)$ to avoid overfitting issue.

\section{Nonstationary Multivariate Gaussian Processes (NMGP)}
To model the essence of nonstationarity, the literature can be summarized into two categories. One category is to propose a nonstationary model such as a mixture of Gaussian processes \cite{tresp2001mixtures}, infinite mixtures of Gaussian process experts \cite{rasmussen2002infinite}, warped Gaussian processes, and treed Gaussian process \cite{gramacy2008bayesian}. The other category is to extend stationary kernel to the corresponding nonstationary kernel. Gibbs proposed a Gibbs kernel by extending the RBF kernel with input-dependent length-scales in \cite{gibbs1998bayesian}. It is extended to different types of multivariate kernels in \cite{paciorek2004nonstationary} motivated by covariance function construction in \cite{higdon1999non}. By assign input-dependent signal variance, \cite{tolvanen2014expectation, heinonen2016non} discuss the inference on this kind of nonstationary kernels.

Here we consider input-dependent signal variance and input-dependent length-scale in the standard RBF kernel for $K$, the same as proposed in \cite{heinonen2016non}. In our model, it contributes to the ability to model the varying scale and varying change rate across time. Mathematically, the kernel is given by:
\begin{align}
    k(t, t')  & = & \sigma(t)\sigma(t') \sqrt{\frac{2\ell(t)\ell'(t)}{\ell(t)^2 + \ell(t')^2}}\exp\left(-\frac{(t-t')^2}{\ell(t)^2 + \ell(t')^2}\right)
    \label{formula:non_kernel}
\end{align}
It is a special case of the Generalized Spectral Mixture (GSM) kernel \cite{remes2017non}, when considering a one component $Q = 1$ mixture and the frequency function is set to be a constant $\mu(x) \equiv 0$.

We employ a log Gaussian process prior for the scale function $\sigma(t)$ and length-scale function $\ell(t)$ such that
\begin{align}
    & \tilde{\ell}(t) \equiv \log(\ell(t)) \sim \mathrm{GP}(\mu_{\tilde{\ell}}, K_{\tilde{\ell}}(t, t')) \nonumber \\
    & \tilde{\sigma}(t) \equiv \log(\sigma(t)) \sim \mathrm{GP}(\mu_{\tilde{\sigma}}, K_{\tilde{\sigma}}(t, t')) 
\end{align}

However, this NMGP assumes that the correlation across output dimensions is invariant across time, since it employ the separable structure for covariance modeling. To model varying correlation of output dimensions, we propose a generalized nonstationary multivariate Gaussian process in the next section. 

\section{Generalized Nonstationary Multivariate Gaussian Processes (GNMGP)}
To model the varying correlation, we introduce the spatially varying linear model \cite{gelfand2004nonstationary} by considering input-dependent $\bm L(t)$. It can be expressed as
\begin{align}
    & \bm y(t) = \bm L(t)\bm g(t) + \bm \epsilon(t), \qquad \bm\epsilon(t) \sim \mathcal{N}(0, \sigma^2_{err}I) \nonumber \\
    & g_d(t) \stackrel{iid}{\sim} \mathrm{GP}(0, K) 
    \label{formula:SVLMC}
\end{align}
Instead of modeling the matrix-variate inverse Wishart spatial process $\bm B(t)$, we directly put independent identical Gaussian process priors on each entry $L_{ij}(t)$ for $i\geq j$. Therefore
\begin{align}
    L_{ij}(t) \sim \mathrm{GP}(\mu_L, K_L(t, t')) \qquad i\geq j\,.
\end{align}
In this case, due to (\ref{formula:SVLMC}), the covariance function is 
\begin{align}
    K^f(t, t', m, m') & = [\bm L(t)\mathrm{cov}(\bm g(t), \bm g(t'))\bm L^T(t')]_{mm'} \nonumber \\
    & = K(t,t')[\bm L(t)\bm L^T(t')]_{m,m'}
    \label{formula:kernel_GNMGP}
\end{align}
In order to guarantee model identifiability for the scale, we employ the gibbs prior instead of (\ref{formula:non_kernel}), where the scale function $\sigma(t)$ is fixed as the identity function. Otherwise, $\bm L(t)$ is not identifiable.



\section{Properties of the GNMGP}

\subsection{Relation to our Nonstationary Multivariate Gaussian Processes}
We confirm that the proposed generalized nonstationary multivariate Gaussian processes reduce to the proposed nonstationary multivariate Gaussian processes with appropriate parameterization. 

Given (\ref{formula:kernel_GNMGP}), the proposed multivariate covariance function for GNMGP is
\begin{align}
    K^f(t,t') & = \mathrm{cov}(\bm f(t), \bm f(t')) \\
    & = 
    \sqrt{\frac{2\ell(t)\ell'(t)}{\ell(t)^2 + \ell(t')^2}}\exp\left(-\frac{(t-t')^2}{\ell(t)^2 + \ell(t')^2}\right)\bm B(t, t')
\end{align}
where $\bm B(t, t') = \bm L(t)\bm L^T(t')$. The proposed multivariate covariance function for NMGP is
\begin{align}
    & K^f(t, t') = \sigma(t)\sigma(t') \sqrt{\frac{2\ell(t)\ell'(t)}{\ell(t)^2 + \ell(t')^2}}\nonumber \\
    & \qquad \exp\left(-\frac{(t-t')^2}{\ell(t)^2 + \ell(t')^2}\right)\bm B\,.
\end{align}
If we assign the following functions $\bm L(t) = \sigma(t)\bm L$ for the GNMGP, we retrieve the NMGP. 

\subsection{Relation to other Nonstationary Multivariate Gaussian Processes}
\cite{heinonen2016non} proposed a fully nonstationary univariate kernel (\ref{formula:non_kernel}). Our proposed kernel for the NMGP extends it to a multivariate kernel via a separable structure and our proposed kernel for the GNMGP extends it to a multivariate kernel via a nonseparable structure. 

\cite{gelfand2004nonstationary} proposed a nonstationary model via considering a spatially varying covaraince relation but did not emphasize the input-dependent length-scale, which is crucial in real applications.

\cite{paciorek2004nonstationary} proposed a class of non-stationary kernels as follows:
\begin{align}
    & K^{NS}(\bm x_i, \bm x_j) = |\Sigma_i|^{1/4}|\Sigma_j|^{1/4}|(\Sigma_i + \Sigma_j)/2|^{-1/2}R^S(\sqrt{Q_{ij}}) \nonumber \\
    & Q_{ij} = (\bm x_i - \bm x_j)^T((\Sigma_i + \Sigma_j)/2)^{-1}(\bm x_i - \bm x_j)
\end{align}
where $R^S(\cdot)$ is a stationary positive definite kernel. This model considers the univariate output but multivariate input case, especially with a Mat\'ern kernel for $R^S(\cdot)$. Extension of our models with the Mat\'ern kernel is straightforward. 

%%%%%%%%%%%%%%%%%
\begin{comment}
%%%%%%%%%%%%%%%%%

They share the same log likelihood such that
\begin{align*}
    \ell = \log\mathcal{N}(\vec{\bm y}|0, \bm B\otimes \bm K + \sigma^2_{err}I)
\end{align*}
where $\bm B = \bm L^T\bm L$.

The prior of $\sigma^2_{err}$ and $\bm L$ are given as
\begin{align}
    & \sigma^2_{err} \sim \mathrm{IG}(a, b)\,, \nonumber \\
    & L_{ij} \sim \mathcal{N}(0, c) \qquad i\geq j\,.
\end{align}
We put a non-informative prior for $\sigma$ such that $\log\sigma \propto 1$ and an informative prior for length-scale parameter $\ell$ such that $\log\ell \sim \mathcal{N}(0, s)$ to avoid overfitting issue.

%%%%%%%%%%%%%%%%
\end{comment}
%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%
\begin{comment}
%%%%%%%%%%%%%%%%%

To model the varying correlation, we introduce the spatially varying linear model \cite{gelfand2004nonstationary} by considering input-dependent $\bm L(t)$. It can be expressed as
\begin{align}
    & \bm y(t) = \bm L(t)\bm g(t) + \bm \epsilon(t), \qquad \bm\epsilon(t) \sim \mathcal{N}(0, \sigma^2_{err}I) \nonumber \\
    & g_d(t) \stackrel{iid}{\sim} \mathrm{GP}(0, K) 
    \label{formula:SVLMC}
\end{align}
Instead of modeling the matrix-variate inverse Wishart spatial process $\bm B(t)$, we directly put independent identical Gaussian process priors on each entry $L_{ij}(t)$ for $i\geq j$. Therefore
\begin{align*}
    L_{ij}(t) \sim \mathrm{GP}(\mu_L, K_L(t, t')) \qquad i\geq j\,.
\end{align*}
In this case, due to (\ref{formula:SVLMC}), the covariance function is 
\begin{align}
    K^f(t, t', m, m') & = [\bm L(t)\mathrm{cov}(\bm g(t), \bm g(t'))\bm L^T(t')]_{mm'} \nonumber \\
    & = K(t,t')[\bm L(t)\bm L^T(t')]_{m,m'}
    \label{formula:kernel_GNMGP}
\end{align}
In order to guarantee model identifiability for the scale, we employ the gibbs prior instead of (\ref{formula:non_kernel}), where the scale function $\sigma(t)$ is fixed as the identity function. Otherwise, $\bm L(t)$ is not identifiable.

%%%%%%%%%%%%%%%%
\end{comment}
%%%%%%%%%%%%%%%%





%%%%%%%%%%%%%%%%%
\begin{comment}
%%%%%%%%%%%%%%%%%

Here we consider input-dependent signal variance and input-dependent length-scale in the standard RBF kernel for $K$, the same as proposed in \cite{heinonen2016non}. In our model, it contributes to the ability to model the varying scale and varying change rate across time. Mathematically, the kernel is given by:
\begin{align}
    k(t, t')  & = & \sigma(t)\sigma(t') \sqrt{\frac{2\ell(t)\ell'(t)}{\ell(t)^2 + \ell(t')^2}}\exp\left(-\frac{(t-t')^2}{\ell(t)^2 + \ell(t')^2}\right)
    \label{formula:non_kernel}
\end{align}
It is a special case of the Generalized Spectral Mixture (GSM) kernel \cite{remes2017non}, when considering a one component $Q = 1$ mixture and the frequency function is set to be a constant $\mu(x) \equiv 0$.

We employ a log Gaussian process prior for the scale function $\sigma(t)$ and length-scale function $\ell(t)$ such that
\begin{align*}
    & \tilde{\ell}(t) \equiv \log(\ell(t)) \sim \mathrm{GP}(\mu_{\tilde{\ell}}, K_{\tilde{\ell}}(t, t')) \nonumber \\
    & \tilde{\sigma}(t) \equiv \log(\sigma(t)) \sim \mathrm{GP}(\mu_{\tilde{\sigma}}, K_{\tilde{\sigma}}(t, t')) 
\end{align*}

However, this NMGP assumes that the correlation across output dimensions is invariant across time, since it employs the separable structure for covariance modeling. To model varying correlation of output dimensions, we propose a generalized nonstationary multivariate Gaussian process in the next section. 

%%%%%%%%%%%%%%%%%
\end{comment}
%%%%%%%%%%%%%%%%%




\subsection{Relation to other models}
%\subsubsection{Relation to our Nonstationary Multivariate Gaussian Processes}

The proposed GNMGP model can be understood as generalizations of existing GP models. For example,  \cite{gelfand2004nonstationary} proposed a nonstationary model by considering a spatially varying covaraince relation but did not emphasize the input-dependent length-scale, which is crucial in real applications. 
When using a matrix-variate inverse Wishart spatial process for the covariance matrix $\bm B(t) = \bm L^T(t) \bm L(t)$ and a stationary kernel, such as the RBF kernel, for the temporal kernel $K$,  our model reduces to the spatially varying linear model. 

%We confirm that the proposed generalized nonstationary multivariate Gaussian processes reduce to the proposed nonstationary multivariate Gaussian processes with appropriate parameterization. 

\cite{heinonen2016non} proposed a fully nonstationary univariate kernel in (\ref{formula:non_kernel}). Our proposed kernel for the separable GNMGP model extends is a multivariate extension of this model. Given (\ref{formula:kernel_GNMGP}), the proposed multivariate covariance function for GNMGP is
\begin{align*}
    K^f(t,t') &= \mathrm{cov}(\bm f(t), \bm f(t')) \\
    &= 
    \sqrt{\frac{2\ell(t)\ell'(t)}{\ell(t)^2 + \ell(t')^2}}\exp\left(-\frac{(t-t')^2}{\ell(t)^2 + \ell(t')^2}\right)\bm B(t, t')
\end{align*}
where $\bm B(t, t') = \bm L(t)\bm L^T(t')$. Our proposed separable multivariate covariance function is
\begin{align*}
    & K^f(t, t') = \sigma(t)\sigma(t') \sqrt{\frac{2\ell(t)\ell'(t)}{\ell(t)^2 + \ell(t')^2}} \\
    & \qquad \exp\left(-\frac{(t-t')^2}{\ell(t)^2 + \ell(t')^2}\right)\bm B\,.
\end{align*}
If we assign the following functions $\bm L(t) = \sigma(t)\bm L$ for the GNMGP, we retrieve the NMGP. 

%\subsubsection{Relation to other Nonstationary Multivariate Gaussian Processes}

%\textbf{Do we need this next paragraph? I'm not really sure how this relates to our mode?}
Finally we note that using different kernel functions  can offer extensions to other models as well. For example, \cite{paciorek2004nonstationary} proposed a class of non-stationary kernels  
%as follows:
%\begin{align*}
%    & K^{NS}(\bm x_i, \bm x_j) = |\Sigma_i|^{1/4}|\Sigma_j|^{1/4}|(\Sigma_i + \Sigma_j)/2|^{-1/2}R^S(\sqrt{Q_{ij}}) \nonumber \\
%    & Q_{ij} = (\bm x_i - \bm x_j)^T((\Sigma_i + \Sigma_j)/2)^{-1}(\bm x_i - \bm x_j)
%\end{align*}
%where $R^S(\cdot)$ is a stationary positive definite kernel. 
for univariate output with a Mat\'ern kernels.
 %When considering the univariate input case and multivariate output case, 
 Extensions of our model to the Mat\'ern kernel is straightforward, providing a multivariate output alternative to the model in \cite{paciorek2004nonstationary}.
 
 
 
 
 
 
 
 

\subsection{Separable Nonstationary Multivariate Gaussian Process}
In general the above model will be nonseparable, meaning the covariance function cannot be decomposed into components that are functions of either time or dimension, but not both.  In this section we derive a special case of the above model that is separable. 




\cite{heinonen2016non} proposed a fully nonstationary univariate kernel by extending the standard Gibbs kernel to include input-dependent signal variance and input-dependent signal noise. Similar to their univariate kernel we propose the following temporal kernel for our model. 
%\begin{align}
%    K(t, t')  & = & \sigma(t)\sigma(t') %\sqrt{\frac{2\ell(t)\ell(t')}{\ell(t)^2 + %\ell(t')^2}}\exp\left(-\frac{(t-t')^2}{\ell(t)^2 + %\ell(t')^2}\right).
%    \label{formula:non_kernel}
%\end{align}
%\begin{align}
%    K(t, t')  =  \sigma(t)\sigma(t') %\frac{\sqrt{2\ell(t)\ell'(t)}}{\theta(t, t') %}e^{-\left(\frac{t-t'}{\theta(t, t') }\right)^2},
%    \label{formula:non_kernel}
%\end{align}
%where $\theta(t, t') = \sqrt{\ell(t)^2 + \ell(t')^2}$.
\begin{align*} %\label{formula:non_kernel}
    K(t, t') &=\sigma(t)\sigma(t') \sqrt{\frac{2\ell(t)\ell(t')}{\ell(t)^2 + \ell(t')^2}}e^{-\frac{(t-t')^2}{\ell(t)^2 + \ell(t')^2}}, \\
\end{align*}
It is a special case of the Generalized Spectral Mixture (GSM) kernel \cite{remes2017non}, when considering a one component $Q = 1$ mixture and the frequency function is set to be a constant $\mu(x) \equiv 0$.

We employ a log Gaussian process prior for the scale function $\sigma(t)$ and length-scale function $\ell(t)$ such that
\begin{align*}
    %& \tilde{\ell}(t) \equiv 
    \log(\ell(t)) &\sim \mathrm{GP}(\mu_{\tilde{\ell}}, K_{\tilde{\ell}}(t, t')),  \\
    %& \tilde{\sigma}(t) \equiv 
    \log(\sigma(t)) &\sim \mathrm{GP}(\mu_{\tilde{\sigma}}, K_{\tilde{\sigma}}(t, t')).
\end{align*}
Plugging this temporal kernel into the above GNMGP model

Our proposed kernel for the separable GNMGP model extends is a multivariate extension of this model. Given (\ref{formula:kernel_GNMGP}), the proposed multivariate covariance function for GNMGP is
\begin{align*}
    K^f(t,t') &= \mathrm{cov}(\bm f(t), \bm f(t')) \\
    &= 
    \sqrt{\frac{2\ell(t)\ell'(t)}{\ell(t)^2 + \ell(t')^2}}\exp\left(-\frac{(t-t')^2}{\ell(t)^2 + \ell(t')^2}\right)\bm B(t, %t')
\end{align*}
where $\bm B(t, t') = \bm L(t)\bm L^T(t')$. Our proposed separable multivariate covariance function is
\begin{align*}
    & K^f(t, t') = \sigma(t)\sigma(t') \sqrt{\frac{2\ell(t)\ell'(t)}{\ell(t)^2 + \ell(t')^2}} \\
    & \qquad \exp\left(-\frac{(t-t')^2}{\ell(t)^2 + \ell(t')^2}\right)\bm B\,.
\end{align*}

Defining $\bm L(t) = \sigma(t)\bm L$ for the GNMGP, we retrieve the NMGP. 


